Edge Intelligence: Paving the Last Mile of Artificial Intelligence with Edge Computing

With the breakthroughs in deep learning, the recent years have witnessed a booming of artificial intelligence (AI) applications and services, spanning from personal assistant to recommendation systems to video/audio surveillance. More recently, with the proliferation of mobile computing and Internet-of-Things (IoT), billions of mobile and IoT devices are connected to the Internet, generating zillions Bytes of data at the network edge. Driving by this trend, there is an urgent need to push the AI frontiers to the network edge so as to fully unleash the potential of the edge big data. To meet this demand, edge computing, an emerging paradigm that pushes computing tasks and services from the network core to the network edge, has been widely recognized as a promising solution. The resulted new inter-discipline, edge AI or edge intelligence, is beginning to receive a tremendous amount of interest. However, research on edge intelligence is still in its infancy stage, and a dedicated venue for exchanging the recent advances of edge intelligence is highly desired by both the computer system and artificial intelligence communities. To this end, we conduct a comprehensive survey of the recent research efforts on edge intelligence. Specifically, we first review the background and motivation for artificial intelligence running at the network edge. We then provide an overview of the overarching architectures, frameworks and emerging key technologies for deep learning model towards training/inference at the network edge. Finally, we discuss future research opportunities on edge intelligence. We believe that this survey will elicit escalating attentions, stimulate fruitful discussions and inspire further research ideas on edge intelligence.

==> Makefile <==
# Makefile for LaTeX document files
# Created by Baochun Li, bli@eecg.toronto.edu, March 30 2001
# Modified by Zimu Liu, zimu@eecg.toronto.edu, December 8, 2009
# Last modified: December 8, 2009

# Produce PS/PDF/DVI files: make
# Clean all output files: make clean

# Use pdflatex or latex
ENGINE=pdflatex

# Name of the master LaTeX file
DOCUMENT=main

#--------------------------------------------------
# Do NOT change anything below
#--------------------------------------------------

default: $(DOCUMENT).pdf

$(DOCUMENT).toc: $(DOCUMENT).tex
	$(ENGINE) $(DOCUMENT).tex

ifeq ($(ENGINE), pdflatex)
#--------------------------------------------------
# pdflatex
#--------------------------------------------------
$(DOCUMENT).pdf: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	$(ENGINE) $(DOCUMENT).tex
	$(ENGINE) $(DOCUMENT).tex
else
#--------------------------------------------------
# latex
#--------------------------------------------------
$(DOCUMENT).dvi: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	$(ENGINE) $(DOCUMENT).tex
	$(ENGINE) $(DOCUMENT).tex

$(DOCUMENT).ps: $(DOCUMENT).dvi
	dvips -t letter -Ppdf -G0 -o $@ $<

$(DOCUMENT).pdf: $(DOCUMENT).ps
	cat $(DOCUMENT).ps | ps2pdf - > $(DOCUMENT).pdf 
endif

all: $(DOCUMENT).pdf

clean:
	rm -rf $(DOCUMENT).aux $(DOCUMENT).log $(DOCUMENT).toc \
     $(DOCUMENT).bbl $(DOCUMENT).blg $(DOCUMENT).pdf \
     $(DOCUMENT).ps $(DOCUMENT).dvi


==> application.tex <==
\section{Application of Edge Intelligence}
In this section, we discuss applications enabled by edge intelligence, together with their realistic use cases. %We first summarized these applications in Fig. \ref{}

\begin{table*}[!htb]
	\footnotesize
	\caption{Applications of edge intelligence} \label{eiapp}
		\centering
		\begin{tabular}{l|l|l|l}
			\hline
			EI Application
			& AI Basis
			& Commercial Products
			& Category
			\\\hline\hline
			
			\multirow{5}{*}{Video Analytics}
			& \multirow{5}{*}{CV}
			& SenseTime SenseDLC SDK
			& Software
			\\
			
			&
			& HIKVISION iDS Smart Camera
			& Device
			\\
			
			&
			& Dell EMC Video Surveillance Solution
			& Platform
			\\
			
			&
			& Huawei Video Surveillance Solution
			& Platform
			\\
			
			&
			& Honeywell  Video Surveillance Solution
			& Platform
			\\\hline
			
			\multirow{4}{*}{Cognitive Assistance}
			& \multirow{4}{*}{CV, NLP, SR}
			& Google Lens
			& Device
			\\
			
			&
			& Amazon Alexa
			& Software
			\\
			
			&
			& Microsoft Cortana
			& Software
			\\
			
			&
			& Apple Siri
			& Software
			\\\hline
			
			\multirow{4}{*}{IIoT}
			& \multirow{4}{*}{CV, Robotics}
			& Intel Industrial Automation
			& Platform
			\\
			
			&
			& IBM PMO
			& Platform
			\\
			
			&
			& Alibaba Cloud ET Industrial Brain
			& Platform
			\\
			
			&
			& Simens MindSphere
			& Platform
			\\\hline

			\multirow{4}{*}{Smart Home}
			& \multirow{4}{*}{CV, NLP, SR, Robotics}
			& Intel Smart Home Development Acceleration Platform
			& Platform
			\\
			
			&
			& Huawei Smart Home Solution
			& Platform
			\\

			&
			& Google Home Hub
			& Software
			\\
			
			&
			& Microsoft Home Hub
			& Software
			\\\hline

			\multirow{3}{*}{Precision Agriculture}
			& \multirow{3}{*}{CV, Robotics}
			& DJI Agriculture Drone
			& Device
			\\
			
			&
			& Intel Precision Agriculture Kit
			& Software
			\\
			
			&
			& KAA Smart Farming Solution
			& Software
			\\\hline

			\multirow{3}{*}{Smart Retail}
			& \multirow{3}{*}{CV, NLP, SR, Robotics}
			& Intel Smart Retail Solution
			& Platform
			\\
			
			&
			& Amazon Go
			& Infrastructure
			\\
			
			&
			& JD.com Unmanned Store
			& Infrastructure
			\\\hline
		\end{tabular}
\end{table*}


\subsection{Video Analytics}
Surveillance cameras are now everywhere, and many cities and organizations are deploying unprecedented amounts of cameras for a wide variety of purposes, including public safety, security surveillance, traffic control and planning and factory floor monitoring. By forecast, the shipments of surveillance cameras are expected to grow at more than 20\% compound annual growth rate from 2017 to 2024 \cite{tvs2018}. Driven by the recent advances in computer vision and deep learning, a continuous stream of increasingly accurate DNN models for object recognition (e.g., ResNet152 and VGG-16) have been proposed, enabling video analytics with great potential. However, due to the huge and ever-growing size of video data, analyzing videos on the cloud is no longer practical, due to the concerns on both performance and cost. Specifically, shipping the large volume of video data via the vulnerable WAN to the cloud incurs prohibitive bandwidth cost and unacceptable transmission latency. 

The recent years have witnessed a shift of moving video analytics from the cloud to the edge \cite{zhang2018distributed, ananthanarayanan2017real, hung2018videoedge,jiang2018chameleon,jiang2018mainstream, Yi2017LAVEA, Quan2018Firework}. Apart from reduced monetary cost and transmission latency, edge computing further empowers video analytics with high responsiveness, location awareness and context awareness. These virtues are quite meaningful to mission-critical tasks in many fields. Taking the “Amber Alert” for child abduction in public safely for example, by vehicle recognition, vehicle license plate recognition and face recognition using various connected cameras at the interested regions, edge computing can identify suspects and suspicious vehicles or persons with the quickest responses \cite{zhang2018distributed}. Due to the great potential of edge-based live video analytics, it is recognized as the “killer application” of edge computing by Microsoft \cite{ananthanarayanan2017real}. More excitingly, realistic deployments of edge-based video analytics have been conducted in cities like Bellevue, WA, Washington, DC, Cambridge in UK, Beijing and Hangzhou in China.  

\textbf{Use Cases}: In partnership with the City of Bellevue, WA, and City of Washington, DC, Microsoft has developed traffic control solutions for the two cities, based on traffic video analytics running on top of edge clusters. By understanding volumes of cars, buses, trucks, motorcycles, bicycles, walkers and near-miss collisions, they proposed solution predicts where future crashes are likely to occur. Actuation systems could then take corrective action (e.g., traffic light duration control) to prevent the collisions. 

\subsection{Cognitive Assistance}
Digital experiences enhanced by cognitive assistance are considered to be among the most promising trends in consumer electronics, as demonstrated by Apple Siri, Google Lens, Microsoft Cortona and Amazon Alexa. Cognitive assistance brings AI technologies such as speech recognition, emotion detection, computer vision and natural language processing within the inner loop of human cognition and interaction. By analyzing sensor data from a wearable device to or a smartphone in a real-time manner, cognitive assistance performs a task required by the users, or returns just-in-time task-specific guidance to the user. For example, Apple Siri can automatically make a phone call based on the voice command of the user. Microsoft Cortona can remind and direct the user to drive to the airport in advance, based on the email of the flight ticket order. With the on-device camera, Google Lens enables visual search by recognizing the interested objects (e.g., a beautiful clothe in the behind the show window) in the camera view and rendering related information. 

With cognitive assistance, many tasks that only humans used to be able to do can be undertaken by wearable or mobile devices. This greatly enriches people's life style, improves human production efficiency, and brings unlimited opportunities for business. A distinctive feature of cognitive assistance is that they are highly interactive and thus requires low latency. However, since cognitive assistance applications typically performs both computational- and data-intensive AI tasks (e.g., vision and audio processing), neither local execution nor cloud offloading is an ideal solution for implementation. Specifically, running on resource- and power-constrained mobile or wearable devices prolongs the data processing time while running on the cloud prolongs the data transmission time. Currently, an emerging class of interactive cognitive assistance applications are poised to edge computing infrastructures, becoming the key demonstrators of edge computing \cite{ha2014towards, DBLP:conf/mobisys/ChenJHHAPHS15, DBLP:conf/edge/ChenHWZAWHEPKSS17, guo2018foggycache}.

\subsection{Industrial Internet-of-Things (IIoT)}
Industry 4.0, also known as smart manufacturing or smart industry, is a vogue word representing the current trend of revolution from traditional manufacturing to intelligent manufacturing. An important element of Industry 4.0 is the Industrial Internet-of-Things (IIoT) that interconnected sensors, instruments, and other devices together with industrial production applications. By empowering IIoT with AI and big data capabilities, we can make production systems high accurate and intelligent, which directly leads to increased efficiency and productivity in assembly/product lines, as well as decreased maintenance and operation expenditures. 

For example, for machine diagnosis, we can use computer vision techniques to recognize the shape change and crack that may lead to the shutdown of machines (e.g., mechanical arms and cutting tools) \cite{Shao2016An}. By doing so, we can diagnosis and maintain machines in a proactive manner, this can greatly reduce the downtime of machines, and thus improve the production efficiency. Another example is the manufacture inspection for quality assurance of products \cite{li2018deep, Luckow2017Deep}. Traditionally, this was performed in an artificial manner, i.e., by hiring inspectors. Today, with edge intelligence, this can be done by using cameras to detect the defects or products passed the assembly line, with greatly improved cost-efficiency.

\textbf{Use Cases}: IBM Predictive Maintenance and Optimization (PMO) is an IIoT solution based on Watson IoT Platform Edge. It enables manufacturing organizations to apply edge intelligence to improve quality and maintenance management with minimal cost. Currently, this solution has been applied by Shenzhen China Star Optoelectronics Technology Co., Ltd. to accelerate and automate quality inspection of the produced LCD screens. The technique significantly boosts production quality and throughput, while cutting management and maintenance cost.

\subsection{Smart Home}
Smart home is also known as home automation, a smart home system controls lighting, climate, security, entertainment systems and appliances in an intelligent manner. Nowadays, several smart home appliances that are built on the basis of IoT concept are already commercially available, as exemplified by smart light, internet TV, smart washer, and robot vacuum, etc. However, most of current practices on smart home just equip the electrical devices with wireless communication modules, connect them to the cloud, and enable them with remote control capabilities. Clearly, this is insufficient to fully unleash the potential of smart home. 

With edge computing in a home environment, smart devices can be connected to the edge computing node which can be a gateway or an access point. By aggregating the data generated by various appliance at the edge computing node and analyzing them in a coordinated manner, more sophisticated services can be provided \cite{CAOJie2017AnOSforInternetofEverything, zhiwei18iotj}. For example, to reduce the electricity bill by intelligently scheduling the workload of multiple appliance to exploit the time-varying electricity price. This goal can be achieved by mining the usage pattern of various appliance from the historical data, and then temporally scheduling the workload in a predictive manner to reduce the electricity expenditure, without harming the user experience \cite{DBLP:conf/uic/ZhangWCLWPX17}. Besides, with edge intelligence, cheap wireless sensors and controllers can be deployed to more corners of the house, making fine-grained control of the smart home possible \cite{Jie2017EdgeOS}. For instance, with more temperature sensors deployed, we can set the temperature of air conditioners in different rooms in a fine-grained manner to improve the comfort level, based on the detected activities. Finally, for low-latency appliance such as vision or voice recognition based smart lock, edge intelligence brings fast response to them.

\textbf{Use Cases}: Intel Smart Home Development Acceleration Platform is a software development kit initially available on Intel Quark™ processors, it is designed to connect devices in the home. Empowered by AI capabilities such as speech, vision and cognition, the kit transforms homes from being merely connected to becoming smart, and bring new ways for consumers to interact with home appliances around them. In collaboration with the Amazon Alexa Voice Service, this technique has been integrated into Alexa (a virtual assistant developed by Amazon), bringing the convenience of voice control to any connected home appliance.

\subsection{Precision Agriculture}
Boosted by the growing population and upward social mobility, the food demand is expected to double by 2050. Clearly, if agriculture is to continue to feed the world, it needs to become more productive. Fortunately, that is already beginning to happen. In addition to bio-techniques, data and intelligence techniques are bringing new ways to farmers to increase yields, improve quality and reduce crop damage. These data- and AI-drive techniques are known as precision agriculture. As predicted by the International Food Policy Research Institute, precision agriculture can help us to meet the doubled food demand via increasing farm productivity by as much as 67\% by 2050 and cutting down agricultural losses \cite{DBLP:conf/nsdi/VasishtKWJCSKSS17}.

Today, edge intelligence has been applied to various major aspects of farming to promote precision agriculture. For example, in irrigation water management, edge intelligence can better assess need and availability of soil water level for crop cultivation. Using the time-series of meteorological data sensed by underground sensors, the future soil moisture level can be predicted using AI methods such as LSTM and DNN, then proactive and precise irrigation can be performed in advance \cite{Mohapatra2018Neural}. Another example is the prevention diseases and pests. Using agricultural drones to scanning crops with visible and Infrared (IR) light, a precise crop image can be constructed during the flying. Then, by analyzing the image with computer vision techniques, we can detect which plants may be infected by bacteria or fungus, helping to prevent disease from spreading to other crops. In addition, edge intelligence can be also applied to crop detection and classification \cite{Bosilj2018Analysis}, detection of fruit stages (raw or ripe) \cite{sa2016deepfruits}, automated harvesting, etc.

\textbf{Use Cases}: Baidu Intelligent Edge (BIE) is an open-source computing platform aimed at environmental detection tasks for cars, drones, and other moving systems. As major component of BIE, the object recognition module BIE-AI-Board is compact enough to be embedded into cameras, drones, robots, and other edge devices. Early partnership with an agricultural drone company has applied this technique to intelligent crop damage detection, the results is quite inspiring —  reducing the usage of pesticide by up to 50 percent.

\subsection{Smart Retail}
In today’s fiercely competitive marketplace of retail, traditional bricks-and-mortar stores need to find new opportunities to improve efficiency, reduce cost and enhance shopping experience. A recent shift towards these goals is smart retaining, this is a term used to describe a set of smart technologies that are designed to give the consumer a greater, faster, safer and smarter experience when shopping. To enable smart retail, IoT technique that tracks information of products and users, AI approach that analyze the acquired user and product data are very essential. 

Edge intelligence is able to improve all the aspects of retailing, ranging from marketing, payment, inventory and cost management to layout optimization, etc. Let’s use a simple and realistic example to show how edge intelligence can transform the retailing industry. When Alice is approaching the geographical reach of a smart shop, proximity-activated promotion would push notifications to her smartphones. If Alice then passes by the smart shop, augmented reality would capture her and deliver the personalized experience of recommended products to her. Next, if Alice really stepped into the shop, a shopping robot may ask about her interested products and direct her to corresponding shelf. Meanwhile, the cameras in the store detect which item she takes or places back the shelf and compute the payment. Then, after Alice pays online and leaves the shop without being checked out by a cashier, the central controller may turn down the lighting and HAVC systems to reduce the energy cost. Finally, by further mining the shopping data, we can predict the popularities of various products, this helps to improve the layout of products and inventory efficiency.  

\textbf{Use Cases}: As a basic realization of smart retail, unmanned store is taking off in China's retail market. The internet giants Alibaba, Tecent and JD.com each opened unmanned stores since 2017. Powered by smart shelves, sensors, cameras, digital signages and cashier-less checkout counters, these stores offer an unprecedented level of convenience for customers – they can simply pick up whatever they want and walk straight out of the store without getting slowed down by queues or payments. 

Beyond the above emerging applications, we should note that \emph{edge intelligence is increasingly boosting many other applications in various vertical areas, such as autonomous driving \cite{zhang2018openvdap, Huang2017Mobile}, smart heathcare \cite{Chang2018A}, smart city \cite{Hossain2018Improving}, smart grid \cite{He2017Real}, intelligent robots \cite{DBLP:conf/hotedge/ChenFS18}, sport and entertainment \cite{DBLP:conf/nsdi/GowdaDSCYGE17}, etc}. Due to the space limit, we do not introduce the application of edge intelligence in these areas one by one, interested readers are referred to the references therein.   



==> case.tex <==
\section{Case Study}

From the standpoint of edge intelligence,  in this  section, a proposed technical framework for edge intelligence called \textsf{Edgent} is introduced, which shows the effectiveness of enabling low-latency DNN model inference. 

%\hfill mds
% 
%\hfill August 26, 2015
%\subsection{Motivation}
%The DNN-based applications typically require a tremendous amount of computation. Due to the powerful computing capacity, the cloud data center takes responsibility on DNN model training and inference. The input data generated from mobile devices is sent to the remote cloud data center for processing. However, with a cloud-centric approach, the transmission of large amounts of data results in a high end-to-end latency. 

%To alleviate the latency bottleneck caused by the server-based method, with the combination of DNN model partition and model early-exit, the preliminary version of \textsf{Edgent} \cite{Li2018edgeintelligence} is proposed to accelerate DNN model inference on-demand in the static bandwidth environment. To improve the decision-making ability in the dynamic bandwidth environment, \textsf{Edgent} introduces a configuration recording the optimal selection for each bandwidth state and implements an online change point detection algorithm to detect the state transition of the current bandwidth.

\subsection{Framework Overview}
\textsf{Edgent} aims at ensuring efficient real-time DNN model inference performance under dyanmic network bandwidth conditions. Combining two enabling technologies of edge intelligence that are model partition and model early-exit to provide balance between accuracy and latency, \textsf{Edgent} automatically and intelligently selects the optimal exit point and the partition point of a DNN model to maximize the accuracy while satisfying the requirement on the execution latency. Fig. \ref{Edgent Overview} shows the overview of \textsf{Edgent}. \textsf{Edgent} consists of three stages: offline configuration stage, online tuning stage, and co-inference stage.

\begin{figure*}[!ht]
	\centering
	% Requires \usepackage{graphicx}
	\includegraphics[scale=0.5]{fig/dnn_inference/system.pdf}\\
	%\vspace{-10pt}
	\caption{Edgent overview}\label{Edgent Overview}
	%\vspace{-5pt}
\end{figure*}

At the offline configuration stage, \textsf{Edgent} performs two initializations : (1) using BranchyNet technology to train DNN models with various exit points, and thus to enable early-exit. (2) creating the configurations for dynamic bandwidth environments. Each generated configuration includes the configuration map and the branchy DNN model structure.  At run time, the bandwidth between the edge server and the mobile device may fluctuate. Thus, for a network bandwidth state, \textsf{Edgent} creates a configuration map to record the optimal selection using a brute force search in an offline manner. To evaluate the performance of each step of  the search, a reward is defined as follow: 
\begin{equation}
reward_{step}=\left\{
\begin{array}{rcl}
\exp^{acc} + throughput & & {t_{step} \leq t_{req}},\\
0 & & {else},
\end{array} \right.
\end{equation}
where $t_{step}$ is the average execution latency in the current search step (i.e., the selected exit point and the partition point in the current search step), which is equal to $1/throughput$. From equation (1), we can see that the search prioritizes that the latency requirement $t_{req}$ should be satisfied. In this case, the requirement is met, the reward is defined as $\exp^{acc} + throughput$, where $acc$ is the accuracy of the exit point used in this step. After comparison, the search returns the highest reward so that the optimal selection under this bandwidth state is found (i.e., given the latency requirement is satisfied, the search emphasizes on improving the accuracy and when multiple options have the similar accuracy, the one with the higher throughput will be selected). Similarly, the optimal selection for other bandwidth states also can be found, therefore, we can build a configuration map which includes the bandwidth state and its optimal selection for device-edge synergy.

At the online tuning stage, the main task of \textsf{Edgent} is to figure out the optimal selection that are the exit point and the partition point, that makes DNN model inference meet latency requirement, using the configuration generated offline. To this end, for the static bandwidth environment, \textsf{Edgent} iteratively searches for the optimal exit point and partition point that makes DNN inference meet latency requirement, using regression models generated offline, for the dynamic bandwidth environment, \textsf{Edgent} implements an online change point detection algorithm \cite{adams2007bayesian} to detect the bandwidth state transition.  The \emph{Optimizer} runs the online change point detection algorithm with the inputs of configuration generated offline, latency requirement and the current bandwidth state. When a bandwidth state transition is detected, the \emph{Optimizer} will search for the bandwidth state which is the closest one to the new bandwidth state in the configuration map and returns the corresponding selections of exit point and partition.

At the co-inference stage, according to the early-exit and partition plan given in the online tuning stage, the edge server will execute the layer before the partition point and the rest will run on the mobile device. 

% needed in second column of first page if using \IEEEpubid
%\IEEEpubidadjcol

\subsection{Performance Evaluation}
The performance of \textsf{Edgent} is evaluated based on the dataset of Belgium 4G/LTE bandwidth logs. As for the  DNN model for testing, a branchy AlexNet with five exit point is trained, of which the number of layers is 12, 16, 19, 20 and 22, respectively. 

Then, \textsf{Edgent} framework runs in the dynamic bandwidth environment emulated by the dataset. 

\begin{figure}[htbp]
	\centering
	% Requires \usepackage{graphicx}
	
	\subfigure[A bandwidth traces on public bus]{
		\includegraphics[scale=0.35]{fig/dnn_inference/bus_0011_trace_logs.pdf}\label{bus trace}
	}
	\subfigure[The throughput of DNN model inference]{
		\includegraphics[scale=0.35]{fig/dnn_inference/bus_0011_tp_logs.pdf}\label{bus throughput}
	}
	\subfigure[The selection of exit point and partition point at each timestamp in the bandwidth traces]{
		\includegraphics[scale=0.35]{fig/dnn_inference/bus_0011_point_logs.pdf}\label{bus selection}
	}
	%	\vspace{-10pt}
	\caption{An example showing the decision-making ability of \textsf{Edgent} in a bandwidth traces on bus}\label{bus result}
	%	\vspace{-10pt}
\end{figure}

Fig. \ref{bus result} shows the experiment result of a bandwidth trace which the transportation is the bus. In Fig. \ref{bus trace}, the bandwidth trace is showed. Fig. \ref{bus throughput} shows the DNN model inference throughput under the bandwidth environment showed in Fig. \ref{bus trace}. And the corresponding optimal selection that the exit point and the partition point of the branchy AlexNet are recorded in Fig. \ref{bus selection}. Seen from the experiment results shown in Fig. \ref{bus result}, the optimal selection of model inference strategy varies with the bandwidth change. The \emph{Optimizer} at online tuning stage works precisely during the dynamic bandwidth environment.

\begin{figure}[H]
	\centering
	% Requires \usepackage{graphicx}
	\includegraphics[scale=0.4]{fig/dnn_inference/tp_comparison.pdf}\\
	\vspace{-5pt}
	\caption{The throughput comparison between two configuration}\label{conf comparison}
	\vspace{-10pt}
\end{figure}

\begin{figure}[H]
	\centering
	% Requires \usepackage{graphicx}
	\includegraphics[scale=0.4]{fig/dnn_inference/reward_comparison.pdf}\\
	\vspace{-5pt}
	\caption{The reward comparison between two configurations}\label{reward comparison}
	\vspace{-10pt}
\end{figure}

And we run the static configuration under the dynamic bandwidth environment, using the Belgium dataset. The static configuration is that we use a regression-based method to estimate the DNN model layer latency to figure out the optimal exit point and partition and the regression models are trained offline. The experiment results are shown in Fig. \ref{conf comparison} and Fig. \ref{reward comparison}.

We record the throughput and the reward under two configuration and calculate the cumulative distribution function of each experiment. Seen from Fig. \ref{conf comparison}, the most part of throughput based on the dynamic configuration is higher than that of throughput based on the static configuration, meaning that under a dynamic bandwidth environment, the \textsf{Edgent} works better with dynamic configuration than with static configuration. As for the result of reward, according to the equation (1), we set the $reward$ to $\exp^{acc} + throughput$ if the latency requirement is met, and then in our experiment, the accuracy of each exit point is 74.7\%, 76.2\%, 76.3\%, 78.1\%, and 78.2\%, respectively. To simplify the calculation of $reward$ and make a better distinction, we use 1.0, 2.0, 3.0, 4.0, 5.0 to indicate the $acc$ of each exit point. The results of the reward are recorded in Fig. \ref{reward comparison}. From the Fig. \ref{reward comparison}, we can see that the most part of reward based on the dynamic configuration is higher than that of reward based on the static configuration, which means that under a dynamic bandwidth environment, the \textsf{Edgent} selects the exit point with higher accuracy when it uses dynamic configuration and when the \textsf{Edgent} uses the static configuration, it may not select the exit point with the higher accuracy and even sometimes selects the collaboration strategy that cannot make inference latency meet the latency requirement.

==> marketplace.tex <==
% by Ke Luo
\section{The Marketplace of Edge Intelligence}
\label{sec:marketplace}

    In this section, we first overview the marketplace of Edge Intelligence and concentrate ourselves on several supporting fields of the EI market. Then we introduce some existing commercial hardware and platforms for EI and characterize them with distinctive features.

	\subsection{Market Overview and Landscape}
	Since EI is the nexus between AI and edge computing, any field that is relevant to AI or edge computing can have a potential impact on the market of EI. However, instead of attempting to grasp the whole market in a few words, we narrow down our view and focus only on fields that are the most critical for EI, namely hardware, software, and platforms on which EI relies. Other market fields like infrastructure, connectivity, traffic routing and delivery, virtualization and containerization, etc. should be orthogonal to EI, and we refer readers to a community-driven state of the edge computing landscape for more details\cite{edge_landscape}.

		\subsubsection{Hardware for EI}
		The most straightforward way to launch EI is to run AI algorithms directly on edge devices. However, as we can expect, edge devices are typically resource-constrained while the latest advanced AI techniques such as DNN models are resource-hungry owing to their complex structures and massive numbers of parameters. Though the workload of AI algorithms poses an obstacle to realizing EI, some startups as well as big companies still see chances in it and have brought AI chips with variant architectures for the edge to the market. Designed for meeting the extreme requirements of heterogeneous edge devices, AI chips for EI are typically purposely optimized for inferencing tasks in a power-efficient manner. The recent years have witnessed more and more startups and big companies stepping into the field of chips dedicated to running AI tasks on resource-constrained devices. Examples include startups like % only AI chips for edge devices should be included
		Cambricon and Horizon Robotics, as well as big companies like Google and Intel, who introduced Edge TPU and Movidius Myriad VPU respectively. A detailed discussion on AI chips for EI is deferred to \S\ref{subsec:ai-chips}.

		\subsubsection{Software for EI}
		Different from the hardware approach that tends to extend the capability of edge devices, there are also efforts on enabling EI in a perspective of software, which can be roughly grouped into two types, namely efforts on reducing the sizes of AI models and on handling the heterogeneity of the architectures of edge devices.
		
		Reducing the sizes of AI models indicates adapting AI models for edge devices with various means as exemplified by parameter binarization and branchy architecture so that the models can better fit the capabilities of edge devices without compromising on performance. Companies focusing on reducing AI model sizes include XNOR.AI, etc.

		Owing to the natural heterogeneity of edge devices, deploying the same AI models onto edge devices can be problematic and requires additional labors. To ease the deployment of AI models on edge devices, there needs an abstraction layer such as containerization for edge runtime so that AI models can be deployed in a hardware-agnostic manner. Projects or companies focusing on the heterogeneity of edge devices include balenaOS, etc.

		\subsubsection{Platforms for EI}
		Besides running AI tasks purely on edge devices with the help of energy-efficient yet powerful AI chips and models tailored for edge devices, there are alternatives for achieving EI which follow the computing paradigm of edge computing and edge-cloud computing, i.e., delegating the computation-intensive AI tasks to nearby edge servers and further offloading tasks to powerful remote cloud when appropriate.

		There are Edge PaaS companies which provide AI-powered edge platforms, so-called platforms for EI, such as Google Cloud IoT Edge and FogHorn. A detailed discussion on platforms for EI is shown in \S\ref{subsec:ei-platforms}.

	\subsection{Emerging Commercial Platforms for EI}\label{subsec:ei-platforms}
	In this subsection, we would first introduce a list of features for EI platforms, and then give some examples and classify existing commercial platforms for EI based on these features.

		\subsubsection{Features for EI Platforms}
		We propose a list of features for EI platforms and if a platform meets all of these features, we regard it as a general EI platform.

		\textbf{Features inherited from IoT platforms.}
		% better if there are references
		Since IoT has become a top-level scenario and is no doubt one of the biggest data generators that can benefit much from both edge computing and AI techniques, we argue that a general EI platform should first be capable of managing a massive number of IoT devices. The features required by an IoT platform usually include supports for real-time responding at the device-side; offline or intermittent-connectivity; multi-layered security of device data, communication within local devices, and communication between local devices and the cloud; cloud-based data aggregation, management, and analytics; and device management and maintenance at scale.

		\textbf{Flexible Cloud-Edge-Device synergy.}
		This is the feature required by edge computing where (partial) compute happens at or in proximity to the sources of data, which is beneficial to enabling real-time responding and filtering out unnecessary data transmission. More specifically, the support for local compute and edge-cloud synergy should be flexible and general since edge devices are naturally heterogeneous, which is to say, are of different architectures, as well as variant computation capacities, storage sizes, power supplies, etc.

		\textbf{Explicit support for AI techniques.}
		This feature is posed by EI, of course, and the intelligence can be achieved at the edge side, at the cloud side, or both.

		In the following, we would give an example of general commercial EI platforms, an example of EI platforms dedicated for some specific applications, and at last, a table of existing EI platforms.

		\subsubsection{An Example of General EI Platforms}
		We shortly introduce Google Cloud IoT Edge, which meets all the features proposed for EI and is so-called a general platform. Logically\footnotemark, the Google Cloud IoT Edge platform can be seen as a combination of three layers, namely the sensors layer, the edge layer, and the cloud layer. The sensors layer is responsible for sensing the environment while the edge layer gathers data from sensors and performs AI-powered analytics to enable intelligent decision making locally in no time. The data collected by edge devices are further uploaded to the remote cloud so that the ML models can be trained incrementally and the configuration of the system can be tuned with new data. Besides, the platform has special support for Edge TPU, an AI chip for EI provided by Google, in its edge runtime and management of a massive number of IoT devices is also supported. An illustration of the architecture of Google Cloud IoT Edge platform is shown in Figure~\ref{fig:google-cloud-iot-edge}.
		
		\footnotetext{Sensors and edge devices need not be separated physically.}
		
		\begin{figure}[!htb]
			\centering
			\includegraphics[width=0.9\linewidth]{fig/google-cloud-iot-edge.pdf}
			\caption{The architecture of Google Cloud IoT Edge platform}
			\label{fig:google-cloud-iot-edge}
		\end{figure}
		
		\subsubsection{An Example of Dedicated EI Platforms}
		We take Huawei's video surveillance platform, which enables intelligent video surveillance via edge-cloud synergy, as an example of dedicated EI platforms. At the edge side, Huawei's AI-enabled software-defined cameras, the M\slash{X} series, use deep learning based computer vision technologies to analyze a large amount of video in real time. The analytics helps extract valuable information from the video and alleviates the pressure of both the network and the cloud. Therefore, the cloud video nodes can handle more cameras and focus on higher-level applications such as video searching among multiple sites.
		
		\subsubsection{Commercial EI Platforms}
		A classification of existing EI platforms is shown in table~\ref{tab:ei-platforms}.
		
		\begin{table}[!htb]
			\caption{Commercial Platforms for EI}\label{tab:ei-platforms}
			\begin{tabular}{@{}p{1.5cm}|p{2.5cm}|p{4cm}@{}}
				\hline
				
				Type
				& Use-case
				& EI platforms
				\\\hline\hline
				
				General
				& \begin{itemize}[
						\setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}
						\setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}
						\setlength{\listparindent}{\parindent}
					]
					\item Industrial IoT
					\item Intelligent V2I
					\item Smart City
					\item Unmanned Retail
				\end{itemize}
				& \begin{itemize}[
						\setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}
						\setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}
						\setlength{\listparindent}{\parindent}
					]
					\item Aliyun Link Edge
					\item AWS IoT with Greengrass
					\item Baidu OpenEdge
					\item FogHorn
					\item Google Cloud IoT Edge
					\item Huawei Intelligent EdgeFabric
					\item IBM Watson IoT Platform
					\item Microsoft Azure IoT Edge
					\item Predix
					\item Smartiply IoT Platform
				\end{itemize}
				\\\hline
				
				\multirow{2}{*}{Dedicated}
				& Facial Recognition System
				& SenseTime SenseFace Face Recognition Surveillance Platform
				\\\cline{2-3}
				
				&
				Video Surveillance
				& Huawei Video Surveillance Platform
				\\\hline
				
			\end{tabular}
		\end{table}
		
	\subsection{Emerging Commercial Devices and Hardware for EI}\label{subsec:ai-chips}
	In this subsection, we would give a hierarchy of AI chips characterized by their target scenarios, and then divide some commercial AI chips into these defined levels accordingly.

		\subsubsection{The Hierarchy of AI Chips}
		Targeting different use-case scenarios, AI chips in the market can be roughly divided into three categories, namely wearable, mobile-device, and edge-infrastructure. Their main differences lie on the compute capability and the power budget.
		
		\textbf{AI chips for wearable} such as wristbands typically provide compute capability ranging from 10MOPS to 100GOPS with the power budget of about 10mW. They are usually designed only for inference tasks and can serve models with sizes ranging from 10KB to 100KB.
		
		\textbf{AI chips for mobile-device} such as IoT devices, smartphones, and mobile VR\slash{AR} devices typically deliver compute capability ranging from 1TOPS to 10TOPS with the power budget of about 1W. AI chips for edge-devices can serve models with sizes about 10MB.

		\textbf{AI chips for edge-infrastructure} typically deliver compute capability starting from 10TOPS with the power budget exceeding 10W. AI chips for edge-infrastructure often have full support for variant inference tasks offloaded from resource-constrained wearable or mobile devices.
		
		\subsubsection{Commercial AI Chips in Hierarchy}
		Table~\ref{tab:ai-chips} summarizes a list of representative commercial AI chips and SoCs, which are divided into different levels according to the hierarchy and further characterized by detailed use-case scenarios.
		
		\noindent\begin{minipage}{\linewidth}
			\vspace{1em}\small
			\centering
			\captionof{table}{Commercial AI chips for EI}\label{tab:ai-chips}
			
			\begin{tabular}{@{}p{1.5cm}|p{2.5cm}|p{4cm}@{}}
				\hline
				
				Hierarchy
				& Use-case
				& AI Chips
				\\\hline\hline
				
				Wearable
				& \begin{itemize}[
						\setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}
						\setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}
						\setlength{\listparindent}{\parindent}
					]
					\item ECG Analysis
					\item Fall Detection
					\item Intelligent Personal Assistant
				\end{itemize}
				& \begin{itemize}[
						\setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}
						\setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}
						\setlength{\listparindent}{\parindent}
					]
					\item Huami MHS001
					\item Huawei Ascend Nano \& Tiny
					\item Intel Movidius Myriad VPU
				\end{itemize}
				\\\hline

				Mobile-device
				& \begin{itemize}[
						\setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}
						\setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}
						\setlength{\listparindent}{\parindent}
					]
					\item Autonomous Driving
					\item Machine Vision
					\item Robotics
					\item Voice Recognition
				\end{itemize}
				& \begin{itemize}[
						\setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}
						\setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}
						\setlength{\listparindent}{\parindent}
					]
					\item Cambricon-1H\slash{1M}
					\item Google Edge TPU
					\item Horizon Robotics Journey\slash{Sunrise}
					\item Huawei Ascend Lite\slash{Mini}
					\item Intel Movidius Myriad VPU
					\item Intel Mobileye EyeQ
					\item NVIDIA Jetson Modules
					\item Xilinx Zynq SoC and MPSoC Edge Cards
				\end{itemize}
				\\\hline
				
				Edge-infrastructure
				& \begin{itemize}[
						\setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}
						\setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}
						\setlength{\listparindent}{\parindent}
					]
					\item Model Tuning
					\item Offloaded Inference Tasks
				\end{itemize}
				& \begin{itemize}[
						\setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}
						\setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}
						\setlength{\listparindent}{\parindent}
					]
					\item Baidu Kunlun
					\item Huawei Ascend Multi-Mini
					\item Intel Nervana
					\item NVIDIA Tesla P4
				\end{itemize}
				\\\hline
				
			\end{tabular}
		\end{minipage}

==> related.tex <==
\section{Edge Computing}
\label{edge}

In this section, we first review the development history of edge computing and present a brief chronology of the major steps in its evaluation. Then, we discuss existing definitions and various benefits or edge computing.

\subsection{Evolution of Edge Computing}

\begin{figure*}[!t]
	\centering %\vspace{-100pt}
	\includegraphics[width=6.4in]{fig/timeline.eps}
	\vspace{-5pt} \caption{The timeline of the evolution of edge computing}
	\label{timeline} 
\end{figure*}

There is a general consensus that edge computing can be traced back to the late 1990s, when MIT researchers introduced the content delivery network (CDN) \cite{dilley2002globally}, and founded Akamai to commercialize this technique to ease Internet congestion and accelerate web performance. A CDN refers to a  cluster of proxy server nodes in close proximity to end-users of the Internet. By prefetching web contents from remote datacenters and caching them locally, CDN is able to deliver high availability, high performance and content customization (e.g., location-based advertising). Since CDN enables substantial bandwidth savings for content providers, it serves a large portion of the Internet content today, ranging from web objects (text, graphics and scripts) and downloadable objects (media files, software, documents) to streaming media. Around the same time period, researchers in CMU demonstrated the potential of computation offloading for mobile computing. Specifically, by offloading the computation of a speech recognition application to a remote server, they showed how to reduce latency and improve buttery life of resource-limited mobile devices \cite{flinn1999energy}. Later in 2001, they generalized these techniques to the concept of ``cyber foraging'' \cite{satyanarayanan2001pervasive}, for the amplification of exploiting wired hardware infrastructures (referred to as surrogates, e.g., desktop computers) to dynamically augment wireless mobile device’s computing capabilities, via short-range wireless peer-to-peer communication technology. 

In spite of the significance of cyber foraging on improving the performance and energy-efficiency of mobile devices, there are also many practical technical barriers. For example, who would provide the infrastructures for cyber foraging? Where to deploy the infrastructures and how to discover them? How to design the business model for cyber foraging? The emergence of cloud computing in the mid-2000s offers a great answer to these open questions. In particular, in the form of Infrastructure-as-a-Service, major companies, such as Amazon, Microsoft and Google, package computing resources in their mega-scale datacenters into virtual machines that can be ubiquitous accessible to users who have connections to the Internet in an on-demand manner. This makes the cloud  the most appealing infrastructure to be leveraged by mobile devices to argument their resource capacities. With cloud computing, many mobile applications, as exemplified by Apple Siri and Google Assistant offload the computation intensive speech-recognition workload to the cloud for processing,  have opened up a  research field known as mobile cloud computing \cite{dinh2013survey}.

%Fast-forwarding to the late 2000s, applications such as face recognition, speech recognition, and language translation achieved substantial progresses over the past decade, reaching near-human performance and quality. 

Many emerging IoT applications, such as autonomous driving and augmented reality, need intensive computation to accomplish object tracking, content analytics and intelligent decision in a real-time manner, in order to meet the requirements for safety, accuracy, performance and user experience. That is to say, {\em the necessity of real-time  edge intelligence for these IoT applications dictates that decision making should take place right here right now at the network edge.} If enormous amounts of data had to be forwarded on up the chain to  more capable servers that typically live in the cloud for advanced data analysis,  the requirements in terms of high bandwidth and low latency (often  millisecond end-to-end latency) would be extremely demanding and stringent. Needless to say, cloud computing can utilize abundant computing resources for handling complex
tasks, but one significant challenge therein is to meet the stringent low
latency requirement, due to unpredictable network delay in
transporting time-sensitive data traffic through the Internet. 
The utility of mobile cloud computing had been evidenced by some empirical studies conducted by CMU. Specifically, for a highly interactive visualization application Quake-Viz that requires high output frame rate, it is observed that local machine with hardware graphics acceleration brings better smoothness than a remote compute server \cite{lagar2007interactive}. Independently, another empirical study conducted in 2006 also showed that the usability of a highly interactive photo editing application suffers unacceptably even at moderate WAN latency (100 ms round-trip time) and very good bandwidth (100 Mbps) \cite{tolia2006quantifying}. 
As conclusion,   {\em it is expected that a high percentage of IoT-created data will have to be stored, processed and analyzed upon close to, or at the edge of the network}.



To tackle the challenging latency issue in  mobile cloud computing, in October   2008,  Microsoft Researchers, together with researchers from CMU, AT\&T, Intel and Lancaster University, came up with a new computing paradigm  called ``cloudlet''. Different from a cloud which is in the remote network core, a cloudlet can be accessed by nearby mobile devices via low-latency, one-hop, high-bandwidth wireless networks. Thanks to physical proximity, cloudlets can  enable low end-to-end response time for the offloaded mobile applications  \cite{Satyanarayanan2009The}. Later in 2009, they published this cloudlet concept via the paper ``The Case for VM-Based Cloudlets in Mobile Computing,'' which has received more than 2500 citations by the end of 2018. Subsequent works on empirical measurements and prototype implementation for latency-sensitive and compute-intensive applications, conducted in the early 2010s \cite{cuervo2010maui,ha2014towards}, have demonstrated the advantages of cloudlets.

Following the concept of cloudlet, in 2012, Cisco proposed the concept of fog computing \cite{bonomi2012fog}, which refers to the continuum computing infrastructure between end devices and traditional cloud-scale datacenters. Unlike cloudlet which was driven by mobile applications, the primitive of fog computing was IoT applications, e.g., connected vehicles, smart grids and smart cities. In year 2010, Institute of Computing Technology (ICT) of Chinese Academy of Science (CAS) initialed the cloud-sea computing systems project \cite{xu2014cloud}, aiming to augment conventional cloud computing by cooperation and integration of the cloud-side systems and the sea-side systems, where the ``sea-side'' refers to an augmented client side consisting of human facing and physical world facing devices and subsystems. In 2013, Pacific Northwest National Laboratory (PNLL) proposed the term edge computing for the first time. In the 2-page report \cite{12edge}, the motivation and main research areas of edge computing were briefly introduced. 

Since 2014, edge computing has stepped into a fast track of development and promotion, as sketched in Fig. \ref{timeline}. In late 2014, the European Telecommunications Standards Institute (ETSI) created a new Industry Specification Group (ISG) to develop technical standards to tackle the complex questions associated with mobile edge computing, attracting the participation of more than 30 IT companies. In the following year, the Open Edge Computing initiative was launched in by Vodafone, Intel, and Huawei in partnership with CMU and expanded a year later to include more industrial members. Also, in 2015, the Open Fog Consortium was created by Cisco, Microsoft, Intel, Dell, and ARM in partnership with Princeton University, and has since expanded to include many other companies. In 2016, Edge Computing Consortium (ECE) was formed in China, with the position of serving as an industrial cooperative platform to promote open cooperation in the operation technology (OT) and information-communication-technology (ICT) fields, nurture the industry’s best application practices, and advance sound and sustainable development of the edge computing industry. By the end of 2018, more than 200 IT companies around the world joined ECE. In the early 2019, 18 vendors and organizations have signed a cooperation agreement to form the Edge Computing Consortium European, aiming to create a standard reference architecture and technology stack that can be deployed across multiple fields.

The driving force from academia should never be neglected. In October 2016, researchers from Wayne State University (WSU) published the first comprehensive vision paper \cite{shi2016edge} that defined the concept, verified the applications and identified the challenges and opportunities of edge computing. By the end of 2018, this this vision paper had been cited for nearly 700 times. Also in October 2016, the First ACM/IEEE Symposium on Edge Computing (SEC) together with NSF Workshop on Grand Challenges in Edge Computing were co-held in Washington, DC. In June 2017, the First IEEE International Conference on Edge Computing (EDGE) was held in Honolulu, HI. In July 2018, the first USENIX Workshop on Hot Topics in Edge Computing (HotEdge) was held in Boston, MA. Since 2017, workshops on edge computing begun to be held in-conjunction with influential conferences as exemplified by ACM SIGCOMM and IEEE INFOCOM. To further popularize the concept of edge computing to wider rage of audiences, researchers from Wayne State University (WSU), Anhui University, Sun Yat-sen University (SYSU) and Xidian University co-authored the first book about edge computing, which was published by Science Press in January 2018 \cite{shi2018edge}. 

%\begin{figure}[!t]  
%	\centering %\vspace{-100pt}
%	\includegraphics[width=3.8in]{fig/trends.eps}
%	 \caption{Google Trend showing more attention toward edge computing in recent years.}
%	\label{fig-trend} \vspace{-15pt}
%\end{figure}

Realizing the great business opportunities provided by edge computing, a crowd of companies have flooded into the edge computing market. In December 2016, Amazon made foray into edge computing with AWS Greengrass, a service that brings local computing, messaging, data caching, sync, and ML inference capabilities to edge devices. In April 2018, Microsoft announced that it would invest \$5 billion in IoT and edge computing technologies over the next four years. Google has also recently released the edge TPU AI chips and Cloud IoT Edge platform to bolster its edge computing strategy. For the internet giant Baidu from China, it also launched and open-sourced it edge computing platform OpenEdge in 2018. A more comprehensive and holistic profile of the of the marketplace of edge intelligence will be given in Sec. V. In a nutshell, the game change on edge computing between the giant players in the IT sector indicates that edge computing is stepping into a booming era.

\subsection{Definitions and Benefits of Edge Computing}\label{edgebenefits}

Even though the notion of `edge computing' was first introduced in 2013, there is still a lack of a highly recognized definition for edge computing. Specifically, various organizations have defined edge computing from different perspectives.

In 2013, when edge computing was first introduced in a 2-page report \cite{12edge}, Pacific Northwest National Laboratory (PNLL) gave the definition that ``Edge computing is pushing the frontier of computing applications, data, and services away from centralized nodes to the logical extremes of a network. It enables analytics and knowledge generation to occur at the source of the data. This approach requires leveraging resources that may not be continuously connected to a network such as laptops, smartphones, tablets and sensors.'' This definition focuses on the on-premise capability that enables service continuity even without network connection to the cloud. Since at that time, connectivity was not ubiquitously or economically available.  

In 2015, in an introductory technical white paper \cite{hu2015mobile} released by ETSI, mobile edge computing is defined as ``a key technology towards 5G, which provides an IT service environment and cloud-computing capabilities at the edge of the mobile network, within the Radio Access Network (RAN) and in close proximity to mobile subscribers. The aim is to reduce latency, ensure highly efficient network operation and service delivery, and offer an improved user experience.''As a standard organization for telecommunications, ETSI defines edge computing as a technical enabler of the upcoming 5G which requires low latency, and stresses the superiority of edge computing on reducing the latency, and thus improving mobile experience and network operation. Moreover, for the first time, EISI pointed out that the edge node should be placed within the RAN to ensure the physical proximity.


In 2016, in a positioning paper \cite{shi2016edge} published by Wayne State University (WSU), edge computing is defined as ``the enabling technologies allowing computation to be performed at the edge of the network, on downstream data on behalf of cloud services and upstream data on behalf of IoT services. Here ‘edge’ as any computing and network resources along the path between data sources and cloud data centers.'' Clearly, this definition from WSU is highly related to IoT, since the latter has emerged as a top-scenario at that time. With the push of data from cloud services and pull of data from IoT, the edge of the network is changing from data consumer to data producer as well as data consumer. The definition above highlights the potential of edge computing on addressing the concerns of response time requirement, battery life constraint, bandwidth cost saving, as well as data safety and privacy.

As a cloud computing service provider, in 2018, Microsoft defined edge computing as \cite{msedge} ``where compute resources, ranging from credit-card-size computers to micro data centers, are placed closer to information-generation sources, to reduce network latency and bandwidth usage generally associated with cloud computing. Edge computing ensures continuation of service and operation despite intermittent cloud connections.'' By this definition, edge computing is the paradigm that the information-generation source makes use of the available and widely dispersed computing resources for computation, and thus to reduce the network latency and bandwidth usage. The edge node can be varying in size: as smaller as a credit-card-size computer, and as larger as a micro datacenter with several server racks.

\begin{figure}[!t]  
	\centering %\vspace{-100pt}
	\includegraphics[width=3.4in]{fig/edge.eps}
	 \caption{An illustration of edge computing}
	\label{fig-edge} \vspace{-15pt}
\end{figure}

While the detailed definition of edge computing varies from different organizations, physical proximity is the most essential characteristic emphasized by those definitions. To ensure physical proximity, an edge node can be a server attached to an access point (e.g., WiFi, router, cellular tower), a network gateway, or a micro-datacenter in practice, as shown in Fig. \ref{fig-edge}. Besides, D2D (device-to-device) offloading \cite{asadi2014survey} that offloads data or tasks among nearby end-devices also ensures physical proximity and has the virtues of high data rate, energy-efficiency. Therefore, D2D offloading is also generally recognized as a form of edge computing \cite{mao2017survey, chen2017exploiting,wang2017survey}. Notably, the physical proximity between the computing and information-generation sources have several benefits compared to the traditional cloud-based computing paradigm, including low-latency, energy-efficiency, privacy protection, reduced bandwidth consumption, on-premises and location awareness. We next elaborate these benefits as follows.

\textbf{Low-Latency}: Humans are naturally sensitive to delays in the critical path of interaction. For a mobile service, the end-to-end latency perceived by the end-users typically consists of 4 components: data transmission delay, network propagation delay, queuing delay and computing delay \cite{kurose2009computer}. By pushing the computing resources from the remote network core to the network edges that are in very close proximity to the end users, the network propagation delay can be significantly reduced, due to the greatly shortened network distance. Besides, with cloud computing, the information flow is required to pass through multiple network gateways, routers and switches distributed at several networks including the access network, backhaul network and WAN, where traffic control, routing and other network-management operations can contribute to excessive queuing delay. Moreover, in edge computing, the end users can access the edge computing node via metropolitan-area-network (MAN) or local-area-network (LAN) whose bandwidth is typically sufficient and stable. In a sharp contract, in cloud computing, the information should traverse the WAN whose bandwidth are scares, limited and unstable (in terms of jitters) \cite{jalaparti2016dynamic}. This results in much shorter data transmission delay in edge computing than that in cloud computing. Therefore, for mobile applications that do not require excessive amount of computing resource and result in large computing delay, edge computing can significantly reduce the overall end-to-end latency. Extensive recent research efforts have empirical demonstrated the low-latency of edge computing for various mobile applications. For example, for a mobile augmented reality application, CMU showed that cloud computing typically takes 250-1000ms, while edge computing can finish the tasks within 140ms \cite{ha2013impact}. For a mobile face recognition application, researchers from The College of William and Mary observed that edge computing is able to reduce the response time from 900ms to 169ms \cite{yi2015fog}. Undoubtedly, the low latency of edge computing makes it appealing to emerging mission-critical applications as exemplified by augmented reality, interactive game, industrial Internet-of-Things (IIoT) and Internet-of-Vehicles (IoV).

\textbf{Energy-Efficiency}: For mobile and embedded devices, the energy consumption is typically dominated by CPU and network interface that performs computing and data communication, respectively. Due to the limited size of mobile and embedded devices, due to the constraint on the physical size, the capacity of the battery is limited. Therefore, energy efficient task execution is of strategical importance for mobile and embedded devices. Compared to on-device computing, edge computing eliminates the computing energy consumption of the devices. While compared to the cloud computing, edge computing significantly reduces the energy consumption of the network interface incurred by the data transmission, since the transmission delay is greatly reduced as discussed in the last paragraph. Similarly, many empirical measurements have been conducted to compare the energy-efficiency of edge computing and cloud computing. For example, for an augmented reality and a mobile face recognition application, researchers in CMU measured the energy consumption of on-device computing, edge computing, and cloud computing with datacenters in various regions \cite{ha2013impact}. The results are plotted in Fig. \ref{fig-ee}, from which we observe that edge computing has better energy efficiency than on-device computing and cloud computing.

\begin{figure}[!t]  
	\centering %\vspace{-100pt}
	\includegraphics[width=3.4in]{fig/energy-efficiency.eps}
    \caption{The per-operation energy consumption (measured by Jouls) of a face recognition and an argumented reality application on a mobile device,  in which an image from the device is transmitted over a Wi-Fi first hop to an edge node or Amazon Web Services (AWS) datacenters at various regions. }
	\label{fig-ee} \vspace{-15pt}
\end{figure}

\textbf{Bandwidth-Efficiency}: In recent year, Internet-of-Things (IoT) emerged as a top-level scenario. Over the past decade, we have witnessed a wide range of ubiquitous IoT devices as exemplified as surveillance cameras, smart sensors, wearables and Internet-of-Vehicles connected to the Internet. According to forecast of Cisco Visual Networking Index (2017-2022) \cite{ciscovni}, there are an estimated number 18 billion networked devices across the global in 2017, up 22 percent per year, and will reach 28.5 billion by 2022. As a concrete example, the emerging wearable devices have seen a 44.4\% increase in shipments for 2016, compared to the 80 million device shipments in 2015 and the yearly shipments is expected to reach 200 million in 2019 \cite{Seneviratne2017A}. As a result of the booming connectivity, the data volume will grow explosively. By 2020, data generated by the ubiquitous IoT devices worldwide is expected to reach 500 zettabytes, meaning that each person will produce 1.7MB data per second. While in a sharp contrast, the pace of the development of WAN infrastructure that is traditional used to ship the IoT data to the cloud has slowed down \cite{clarinet, vulimiri2015global}. If we still choose to ship the skyrocketing IoT data to the cloud via the WAN infrastructure, we would further exacerbate the pressure faced both the latter. Edge computing is releasing the unprecedented tension faced by the WAN infrastructure now. Specifically, by processing the IoT data at the edge of the WAN, the traffic traversing the WAN can be significantly reduced. As forecasted by IDC, 40\% of IoT-created data will be processed at network edge by 2018 and 50\% by 2025 \cite{shi2016edge}.

\textbf{Privacy Protection}: Compared to cloud computing, the capability of enhancing the privacy and security if the user information is also an attractive advantage owned by edge computing. Specifically, in cloud computing, the infrastructure, i.e., mega-scale datacenters are susceptible to attacks due to their high concentration of information of a big pile of users. Moreover, in cloud computing, the ownership and management of user data are separated, incurring the threat of private data leakage and loss. Fortunately, edge computing brings an effective solution to address the above challenges. Specifically, on one hand, due to the large in number but small in scale nature, the widespread geo-distribution and the less concentration of valuable information, edge servers are much less likely to be attacked by hackers. Besides, while a public cloud is shared by multi-tenants, an edge node can be a private cluster owned by a factory, a company or an organization. This eases the concern of the leakage of user information, since the administrator of the edge cluster fully manages the authorization and access control of service requests, without the need of an external party such as the public cloud. 

\textbf{Context Awareness}: By placing the computing resources and services at the edge of the network, the operator of the edge computing services can leverage low-level signaling information to determine real-time information such as user behaviors, locations, and environments \cite{perera2015context}. This context information allows the delivery of context-aware services to end users, ranging from location-based services to local points-of-interest businesses and network QoS optimization, etc. For example, a retail shopping AR application can benefit not only from knowing the relative location of a user (e.g., the appliance department), but also from knowing that the user is interested in a specific type of appliance (e.g., a microwave oven). Similarly, a video streaming application might optimize its content caching strategy by knowing where the user is and knowing whether a person interacting with the user is someone the user interacted with before \cite{wang2014cache, lobo2014intelligent}.

\textbf{On Premise}: As a local computing unit, edge servers can run  isolated from the rest of the network, while having access to local resources. This becomes particularly important for failure management and defense. If a cloud service becomes unavailable due to network failures, datacenters failures (e.g., power outages) or denial-of-service attacks, the fallback service on the edge can temporarily mask the failure, maintaining the normal operation the services and data. Clearly, this advantage is quite flavored by mission-critical applications (e.g., mobile payment) that suffers great loss due to temporal failures. 





